UWB-ED: Distance Enlargement Attack Detection in Ultra-Wideband

Mobile autonomous systems, robots, and cyber-physical systems rely on accurate positioning information. To conduct distance-measurement, two devices exchange signals and, knowing these signals propagate at the speed of light, the time of arrival is used for distance estimations. Existing distance-measurement techniques are incapable of protecting against adversarial distance enlargement---a highly devastating tactic in which the adversary reissues a delayed version of the signals transmitted between devices, after distorting the authentic signal to prevent the receiver from identifying it. The adversary need not break crypto, nor compromise any upper-layer security protocols for mounting this attack. No known solution currently exists to protect against distance enlargement. We present \textit{Ultra-Wideband Enlargement Detection} (UWB-ED), a new modulation technique to detect distance enlargement attacks, and securely verify distances between two mutually trusted devices. We analyze UWB-ED under an adversary that injects signals to block/modify authentic signals. We show how UWB-ED is a good candidate for 802.15.4z Low Rate Pulse and the 5G standard.

==> sections/Implementation.tex <==
\section{Implementation}
\label{sec:Implementation}



==> sections/charts.tex <==

\newcommand{\wdth}{2.0in}
\newcommand{\hght}{2.0in}
\newcommand{\spcbtwn}{-18 pt}

\begin{figure}
\centering
\subfloat[$n=200$ and $\alpha=50$]{
\label{awelwa7ed}
\begin{tikzpicture}
\begin{axis}[
width=\wdth,
height=\hght,
xlabel=k,
ylabel=Probability,
xmin=0, xmax=200,
ymin=0, ymax=1,
ytick ={0,1},
xtick ={0,100,200},
%extra x ticks={1.5},
extra x tick style={grid=major},
%extra y ticks={0.35,0.54},
extra y tick style={grid=major,yticklabels={,,}},
%minor x tick num=1,
%grid=minor,
tick label style={font=\scriptsize},
x label style={font=\scriptsize,at={(0.5,0.1)}},
y label style={font=\scriptsize,at={(0.31,0.5)}},
legend columns=2,
legend style={draw=none,at={(0.52,0.95)},anchor=north,}
]
\addplot[red] table[col sep=comma]{csv/prob/n200a50r16.csv};
\addlegendentry{\scriptsize r=16}
\addplot[] table[col sep=comma]{csv/prob/n200a50r8.csv};
\addlegendentry{\scriptsize r=8}
\addplot[dashed] table[col sep=comma]{csv/prob/n200a50r4.csv};
\addlegendentry{\scriptsize r=4}
\addplot[dotted] table[col sep=comma]{csv/prob/n200a50r2.csv};
\addlegendentry{\scriptsize r=2}
\addplot[dashdotted] table[col sep=comma]{csv/prob/n200a50r1.csv};
\addlegendentry{\scriptsize r=1}
\end{axis}
\end{tikzpicture}
}
\hspace{\spcbtwn}
\subfloat[$n=100$ and $\alpha=50$]{
\label{tanywa7ed}
\begin{tikzpicture}
\begin{axis}[
width=\wdth,
height=\hght,
xlabel=k,
ylabel=Probability,
xmin=0, xmax=100,
ymin=0, ymax=1,
ytick ={0,1},
xtick ={0,100,200},
%extra x ticks={1.5},
extra x tick style={grid=major},
%extra y ticks={0.35,0.54},
extra y tick style={grid=major,yticklabels={,,}},
%minor x tick num=1,
%grid=minor,
tick label style={font=\scriptsize},
x label style={font=\scriptsize,at={(0.5,0.1)}},
y label style={font=\scriptsize,at={(0.31,0.5)}},
legend columns=2,
legend style={draw=none,at={(0.52,0.95)},anchor=north,}
]
\addplot[red] table[col sep=comma]{csv/prob/n100a50r16.csv};
\addlegendentry{\scriptsize r=16}
\addplot[] table[col sep=comma]{csv/prob/n100a50r8.csv};
\addlegendentry{\scriptsize r=8}
\addplot[dashed] table[col sep=comma]{csv/prob/n100a50r4.csv};
\addlegendentry{\scriptsize r=4}
\addplot[dotted] table[col sep=comma]{csv/prob/n100a50r2.csv};
\addlegendentry{\scriptsize r=2}
\addplot[dashdotted] table[col sep=comma]{csv/prob/n100a50r1.csv};
\addlegendentry{\scriptsize r=1}
\end{axis}
\end{tikzpicture}
}
\caption{Probability of Bin$_\beta$ exceeding Bin$_\alpha$ plotted using equation (\ref{eq:probatksuccesspart1}) in Section~\ref{sec:probfirstcheck}.}
\label{chart:firstcheck}
\end{figure}



































